Faster Walks in Graphs: A $\tilde O(n^2)$ Time-Space Trade-off for Undirected s-t Connectivity

In this paper, we make use of the Metropolis-type walks due to Nonaka et al. (2010) to provide a faster solution to the $S$-$T$-connectivity problem in undirected graphs (USTCON). As our main result, we propose a family of randomized algorithms for USTCON which achieves a time-space product of $S\cdot T = \tilde O(n^2)$ in graphs with $n$ nodes and $m$ edges (where the $\tilde O$-notation disregards poly-logarithmic terms). This improves the previously best trade-off of $\tilde O(n m)$, due to Feige (1995). Our algorithm consists in deploying several short Metropolis-type walks, starting from landmark nodes distributed using the scheme of Broder et al. (1994) on a modified input graph. In particular, we obtain an algorithm running in time $\tilde O(n+m)$ which is, in general, more space-efficient than both BFS and DFS. We close the paper by showing how to fine-tune the Metropolis-type walk so as to match the performance parameters (e.g., average hitting time) of the unbiased random walk for any graph, while preserving a worst-case bound of $\tilde O(n^2)$ on cover time.

==> biblio.tex <==
\begin{thebibliography}{19}

\bibitem{AF}
D.~Aldous, J.~Fill.
\emph{Reversible Markov Chains and Random Walks on Graphs}.
Book draft available at \texttt{http://stat-www.berkeley.edu/users/aldous/RWG/book.html}, 2001.

\bibitem{AKLLR}
R.~Aleliunas, R.M.~Karp, R.J.~Lipton, L.~Lovasz, C.~Rackoff.
Random walks, universal traversal sequences, and the complexity of maze problems. 
\emph{Proc. 20th Annual Symposium on Foundations of Computer Science (FOCS)}, 1979, pp.~218--223.

\bibitem{ACGR}
C.~Alvarez, R.~Greenlaw.
A compendium of problems complete for symmetric logarithmic space.
\emph{Computational Complexity }9:2 (2000), 123--145.

\bibitem{ATWZ}
R.~Armoni, A.~Ta-Shma, A.~Wigderson, S.~Zhou.
An $O(\log(n)^{4/3})$ space algorithm for $(s,t)$ connectivity in undirected graphs.
\emph{Journal of the ACM }47:2 (2000), 294–-311.

\bibitem{BF}
G.~Barnes, U. Feige.
Short random walks on graphs.
\emph{Proc. 25th Annual ACM Symposium of the Theory of Computing (STOC)}, 1993, pp.~728--737.

\bibitem{BBRRT}
P.~Beame, A.~Borodin, P.~Raghavan, W.L.~Ruzzo, M.~Tompa.
Time-Space Tradeoffs for Undirected Graph Traversal by Graph Automata.
\emph{Information and Computation }130:2 (1996), 101--129.

\bibitem{BCERS}
P.~Berenbrink, C.~Cooper, R.~Els\"{a}sser, T.~Radzik, T.~Sauerwald.
Speeding Up Random Walks with Neighborhood Exploration.
\emph{Proc. 21st Annual ACM-SIAM Symposium on Discrete Algorithms (SODA)}, 2010, pp.~1422--1435.

\bibitem{BS}
P.~Berman, J.~Simon.
Lower bounds on graph threading by probabilistic machines.
\emph{Proc. 24th Annual Symposium on Foundations of Computer Science (FOCS)}, 1983, pp.~304--311.

\bibitem{BCDRT}
A.~Borodin, S.A.~Cook, P.W.~Dymond, W.L.~Ruzzo, M.~Tompa.
Two applications of inductive counting for complementation problems.
\emph{SIAM Journal on Computing }18:3 (1989), 559–-578.

\bibitem{BKRU}
A.Z.~Broder, A.R.~Karlin, P.~Raghavan, E.~Upfal.
Trading space for time in undirected $s$-$t$ connectivity.
\emph{SIAM Journal on Computing }23 (1994), 324--334.

\bibitem{CRRST}
A.~Chandra, P.~Raghavan, W.L.~Ruzzo, R.~Smolensky, P. Tiwari.
The electrical resistance of a graph captures its commute and cover times.
\emph{Proc. 21st Annual ACM Symposium of the Theory of Computing (STOC)}, 1989, pp.~574--586.

\bibitem{CR}
S.A.~Cook, C.W.~Rackoff
Space lower bounds for maze threadability on restricted machines.
\emph{SIAM Journal on Computing }9:3 (1980), 630--652.

\bibitem{E}
J.~Edmonds.
Time-space trade-offs for undirected st-connectivity on a JAG.
\emph{Proc. 25th Annual ACM Symposium of the Theory of Computing (STOC)}, 1993, pp.~718--727.

\bibitem{F}
U.~Feige.
A Randomized Time-Space Trade-off of $\O(m\widetilde R)$ for USTCON.
\emph{Proc. 34th Annual Symposium on Foundations of Computer Science (FOCS)}, 1993, pp.~238--246.

\bibitem{GLM}
P.~Gopalan, R.J.~Lipton, A.~Mehta.
Randomized Time-Space Tradeoffs for Directed Graph Connectivity.
\emph{Proc. Foundations of Software Technology and Theoretical Computer Science (FSTTCS)}, LNCS 2914, 2003, pp.~208--216.

\bibitem{HU}
J.E.~Hopcroft, J.D.~Ullman.
Set Merging Algorithms.
\emph{SIAM Journal on Computing }2:4 (1973), 294-–303.

\bibitem{IKY}
S.~Ikeda, I.~Kubo, M.~Yamashita.
The hitting and cover times of random walks on finite graphs using local degree information.
\emph{Theoretical Computer Science }410:1 (2009), 94--100.

\bibitem{Nis}
N.~Nisan.
$RL \subseteq SC$.
\emph{Proc. 24th Annual ACM Symposium of the Theory of Computing (STOC)}, 1992, pp.~619--623.

\bibitem{NOSY}
Y.~Nonaka, H.~Ono, K.~Sadakane, M.~Yamashita.
The hitting and cover times of Metropolis walks.
\emph{Theoretical Computer Science} 411:16--18 (2010), 1889--1894.

\bibitem{Rei}
O.~Reingold.
Undirected connectivity in log-space.
\emph{Journal of the ACM} 55:4 (2008), 1--24.

\bibitem{Sav}
W.J.~Savitch.
Relationships between nondeterministic and deterministic tape complexities.
\emph{Journal of Computer and System Sciences} 4 (1970), 177--192.

\bibitem{SZ}
M.~Saks, S.~Zhou.
$BP_H SPACE(S) \subseteq DSPACE(S^{3/2})$.
\emph{Journal of Computer and System Sciences} 58:2 (1999), 376--403.

\end{thebibliography}
